Predicting digital asset market based on blockchain activity data

Blockchain technology shows significant results and huge potential for serving as an interweaving fabric that goes through every industry and market, allowing decentralized and secure value exchange, thus connecting our civilization like never before. The standard approach for asset value predictions is based on market analysis with an LSTM neural network. Blockchain technologies, however, give us access to vast amounts of public data, such as the executed transactions and the account balance distribution. We explore whether analyzing this data with modern Deep Leaning techniques results in higher accuracies than the standard approach. During a series of experiments on the Ethereum blockchain, we achieved $4$ times error reduction with blockchain data than an LSTM approach with trade volume data. By utilizing blockchain account distribution histograms, spatial dataset modeling, and a Convolutional architecture, the error was reduced further by 26\%. The proposed methodologies are implemented in an open source cryptocurrency prediction framework, allowing them to be used in other analysis contexts.

==> common_content.tex <==
\section{Background}

The following subsections describe the background information for the research.

\subsection{Blockchain and Ethereum}

%is this really needed?
Satoshi Nakamoto's introduction of Bitcoin in November 2008 \cite{bitcoin-paper} has often been hailed as a radical development in money and currency as it's the first example of a digital asset which simultaneously has no backing or ``intrinsic value'' and no centralized issuer or controller. Another arguably more important part of the Bitcoin experiment is the underlying blockchain technology as a tool of distributed consensus. The most important aspect of such technology is the absence of an intermediary (centralized server, bank, company, etc.) between the originator and the recipient, as any changes to the data on this chain are made by consensus among all members of a decentralized network. Thus, avoiding the need to trust third parties. The blockchain can be thought of as a distributed public database with records for each transaction in history. All cryptoasset operations and activity are contained within the blockchain transaction data.

The Ethereum project ($ETH$) is a newer implementation \cite{yellowpaper}, based on the blockchain technology. In addition to the transaction record keeping functionality, Ethereum provides a mechanism for executing program logic on each transaction, thus enabling a much wider variety of use cases of the blockchain technology. Some of which include financial transactions, secure voting, autonomous organizations, company management, freedom of speech networks, online games, crowdfunding, speculation, making it one of the more noisy and difficult to predict blockchains.

\subsection{Autonomous decentralized applications}

The intent of Ethereum is to create an alternative protocol for building autonomous decentralized applications. Because of the blockchain consensus, no one has control over the code execution or storage of these applications. A decentralized application can not be modified outside of the constraints of its logic. Because such an immutable application resembles contractual relations, autonomous decentralized applications are often referred to as ``crypto contracts'', ``smart contracts'' or simply contracts.

\subsection{Transactions and traces}

Every block in the chain is a package of transactions. Every transaction denotes a transfer of value and/or an execution of a smart contract.

Transactions only contain information about the initial (outside) call. For example, if a contract receives funds from $x$ and forwards them to $y$, the transaction will only indicate that the contract received the funds. The transfers the contract additionally makes are known as internal calls. To gather information about them, the initial transaction needs to be replayed in order to observe the derivation from it. Transfers, as well as other contract activity collected using this method are called $traces$.

\subsection{Factors for digital asset value change}

In basic economics, the correlation between supply and demand \cite{supply_demand} determines the price of an asset. Higher demand or lower supply relates to higher price.


Because of small market capitalization, digital currencies are unstable and volatile. Based on our observations of Ethereum, we have identified multiple factors as having a significant influence on the supply and demand of the currency. Most of them can be traced by analyzing the blockchain data in depth.

\subsubsection{Speculative investment}

%PLEASECITATIONNEEDED

Speculative investment is the action of buying and holding a certain asset, speculating that its value will rise in the future. This hampers Ethereum's already low supply and results in artificial price increases.

%In our research, we investigate methods that track the influence of this behaviour to the asset's price.

\subsubsection{Initial Coin Offerings}

Intial Coin Offerings (ICOs) \cite{ico} are share resemblance to Initial Public Offerings, but are implemented using smart contracts and therefore do not bear any of the legal protections that regular investments provide.

During 2017, the total cumulative ICO funding has increased by more than $80$ times \cite{ico-funding}. Ethereum's smart contract framework has become the most targeted platform for ICO fundraising. This is believed to have been a major reason for Ethereum's rise during June 2017.

%We track ICO activities on the blockchain in attempts to observe their impact on value changes.

\subsubsection{Altcoin interference}
\label{altcoin-interference}

After Bitcoin, hundreds of other cryptocurrencies have emerged. Despite the fact that they are completely unrelated and independent from each other, major events in one cryptocurrency can cause unexpected fluctuations in others. For example, major ICO events in Ethereum have caused surges in numerous other currencies, like Litecoin \cite{litecoin}. 

%Currently our prediction models do not take into account the altcoin interference. Our goal is in a further research to include data from other blockchains into our datasets.


%we don't track any such data.
%Should we mention the first sentence? Is it not obvious that it leads to a research ?
%The interference of other alternative coins to Ethereum leads to a whole research topic on its own. We have plans to include historical data and events from other currencies to improve our predictions.

\subsubsection{Media influence}
\label{media-influence}

Crypto market's value can also be easily influenced by media publications. A prime example of this is a case of widespread hoax about an incident with Ethereum's founder Vitalik Buterin \cite{vitalik-death}. This led to temporary plummet and loss of 4\$ billion from Ethereum's market capitalization.

Currently our prediction models do not take into account the media influence. Our goal is in a further research to perform deep-learning based sentiment analysis on news and social media sources related to cryptocurrencies.

%we don't get such data yet, is that a problem?
%In a further research, we will experiment with cases where we track the news stories about Ethereum and similar cryptocurrencies via sentiment analysis.

%\subsubsection{Attacks and thefts}

%Ethereum's smart contract framework is anything but flawless. The immutability and publicity of smart contracts have placed many in concerns that a published contract with flawed code can be attacked and exploited. There have been countless moments of Ethereum's history where similar events have occured. The first major disaster was ``The DAO'' hack, where a hacker stole 50M\$ worth of ETH due to a vulnerability in the contract \cite{dao}. Very recent, and unfortunately much more catastrophic, are two attacks on parity's multi-signature wallet. The first attack was due to a security vulnerability in the contract which resulted in 30M\$ worth of ETH being stolen \cite{parity1}. The second attack happened following the fix of the initial vulnerability, which opened another vulnerability in the process. The result was 300M\$ worth of ETH being completely frozen and unusable, likely forever \cite{parity2}.

%Other than smart contract related attacks, the usual cryptocurrency thefts still stand. Cases where money are sent to the wrong address, someone reveals the private key of an account or simply fools people into sending him ETH for a promise are a common occurrence. There are no consumer protections and no real way to get money returned, if their current owner doesn't want to.

%We will track closely smart contract activity, as well as unusual transfers of tokens to increase our prediction accuracy.



\subsection{Use of Deep Learning in asset value predictions}
Deep Learning \cite{deep_learning} allows for the discovery of patterns in a large dataset. Such a set consists of called dataset samples (forming input-output pairs, such as summarized blockchain activity and the future price). The inputs pass through multiple layers (which perform data transformations with free parameters) and leave as an output. The free parameters have to be set (trained, learned) on known input-output pairs.

Long Short-Term Memory (LSTM) \cite{LSTM} and Convolutional (CNN) \cite{cnn} networks are types of DL networks, which are well known for their performance in time series and image analysis respectively.

\subsubsection{Normalization}
\label{normalization_bg}

%a single value cannot have zero mean and equal variance
Every value in a dataset needs to be normalized (scaled, fit), because of the numerical instability of large computer floating point operations. The general objective for a normalized series is to consist of small numbers of zero mean and equal variance. We use the following normalization algorithms depending on the situation:

$$basic_i = \frac{x_i - min(x)}{(max(x) - min(x))}$$

This basic min-max scale is used to map independent sequences with the same sign to the interval $\in [0; 1]$.

$$around\_zero_i = \frac{x_i + max(\lvert max(x) \rvert, \lvert min(x) \rvert)}{2*max(\lvert max(x) \rvert, \lvert min(x) \rvert)}$$

Similar to $basic$, but maps positive and negative inputs to $(0.5; 1]$ and $[0; 0.5)$ respectively. This scale is used with sequences of varying sign.

%do I need to specify what is std?
$$image_i = (x_i - \frac{1}{n}\sum_{t=1}^{n}x_t) * \frac{1}{std(x)}$$

An an algorithm which produces unbounded time series of zero mean and equal variance. It is used with image-line sequences.
%$$local_i = \frac{win_i}{win_0} - 1$$

%Local normalization based on the first element of a window of values. As it does not depend on the whole sequence, it can normalize future values without issue.
%we don't use sigmoid. Remove it?
%$$sigmoid_i = \frac{1}{1 + \exp(-arr_i)}$$

%Non-linear normalization function that provides consistent normalization no matter the sequence. We recommend this to be used with relatively small values, as normalizing large enough values results in a practically indistinguishable difference in the output value.

\subsubsection{Error measures}
\label{measures}

The following measurement factors are often used to evaluate the performance of predictive DL:

$$
\hspace{2ex}sign = \frac{t}{t+f};
\hspace{2ex}err(t) = out_t - true_t;
\hspace{2ex}null(t) = 0.5 - true_t
$$

$$MSE = \displaystyle\frac{1}{n}\sum_{t=1}^{n}err(t)^2;
\hspace{0.5ex} RMSE = \sqrt{\displaystyle\frac{1}{n}\sum_{t=1}^{n}err(t)^2};
\hspace{0.5ex}R^2 = 1-\displaystyle\frac{\sum_{t=1}^{n}err(t)^2}{\sum_{t=1}^{n}null(t)^2}
$$

%custom = \displaystyle\frac{1}{n}\sum_{t=1}^{n}\frac{\lvert err_t \rvert}{min(pred_t, true_t)};

Where $out$ and $true$ are lists of outputs and expected outputs respectively. If the outputs are binary, then the amount of correctly and incorrectly predicted flags is $t$ and $f$ respectively.

The metrics $R^2$ and $sign$ measure accuracy $\in [0, 1]$, this the aim is to maximize them. In $R^2$ the performance of the model is compared to that of a model always returning the same value. $MSE$ and $RMSE$ are measures of error which have to be minimized.
%In efforts to observe our network's performance from different angles, we have created our own error function, called $custom$.

Traditionally, $MSE$ is used as the loss function during training. The rest are used for performance analysis.

\section{Raw data}
\label{data-sources}

The first kind of data gathered is historical market tick data, which is aggregated from multiple exchanges to achieve a less biased view of the financial state. The frequency (size of each tick) is one hour. Every tick consists of the $open$, $close$, $low$, and $high$ prices, as well as the trade volume to and from the currency for that period. 

The second kind of data is from the Ethereum blockchain. It grows every day \cite{blockchain-size} and includes hundreds of gigabytes worth of transactions, cryptocontract executions, and blockchain events for every moment its existence. For each block in the chain, the following data points are extracted: creation timestamp, number (chain index), miner (block creator), list of confirmed transactions, size in bytes, creation difficulty, and computational resources used (Gas limit and Gas used). The following is stored for each transaction in a block: address of the initiator and receiver, transferred value, used resource units (Gas), and amount paid per resource unit (Gas price). The same kind of information is also collected for internal contract activity by calculating transaction traces.

The total size of the gathered raw blockchain features is around 500GB, containing $5,300,000$ blocks with a total of $194,000,000$ transactions and close to a billion traces. It took 30 consecutive days to download and another 14 to process, filter, format, and save the data to a database.

Both the market and blockchain data are collected for the interval from 8-08-2015 to present.

\section{Generation of data properties}
\label{property-generation}

In order to create a blockchain-based dataset, we first need to extract the most valuable information from the raw blockchain data by performing different feature extraction algorithms. A feature (also called property) is calculated once for each market tick in the historical data in order to form a time series.

We are extracting a set of properties defined in Table \ref{properties}. They are created and selected based on their importance and significance to the prediction problem. A property name with suffix ``$\_rel$'' denotes that its values have been converted to relative ones. An example for a property is seen in Figure \ref{propertyGasUsed}.

\begin{table}[h]
\centering
\begin{tabular}{lp{5.5cm}}
Property & Description \\
\hline
openPrice & The value of ETH at the start of the tick \\
closePrice & The value of ETH at the end of the tick \\
stickPrice & $openPrice - closePrice$ \\
volumeTo & Exchange volume to that cryptocurrency \\
volumeFrom from & Exchange volume from that cryptocurrency \\
transactionCount & Amount of transactions  \\
dappOperations & Amount of transactions to crypto contracts \\
blockSize & The average size of a block in bytes \\
difficulty & The average difficulty for block mining \\
uniqueAccounts & Number of accounts in existence \\
gasLimit & Average limit on computational resource use \\
gasPrice & Average price per gas unit \\
gasUsed & Average amount of gas used \\
networkHashrate & Combined hashrate of every miner in the network \\
ETHSupply & Total amount of Ether in circulation \\
pendingTx & How many transactions per minute are pending for inclusion in the next block \\
blockchainGrowth & Growth of the blockchain size in gigabytes \\
\end{tabular}
\caption{\label{properties}List and description of the properties compiled from the raw data.}
\end{table}

%may be too tiny.
\begin{figure}[h]
\centering\includegraphics[width=\graphwidth]{assets/property_graph}\\
\centering\includegraphics[width=\graphwidth]{assets/property_graph_rel}
\caption{The absolute (up) and relative (down) values of property $gasUsed$ over time. We can observe how major events have influenced the usage of the Ethereum network over time.}
\label{propertyGasUsed}
\end{figure}

The following subsections explain more advanced concepts in calculating properties.

%removing since it isn't used in our experiments
\texcomment{
\subsection{Technical indicators}
Our property values include significant amount of statistical noise which can hamper the training process. We smoothen all of our property values through a set of statistical functions, which are successfully applied in numerous of prediction strategies on the stock market. The functions include Simple Moving Average ($SMA$) and Exponential Moving Average ($EMA$). All of our functions use 10 tick intervals. Property names with suffixes ``$\_sma$'' and ``$\_ema$'' denote that the property values are modified by the respective function. 
}

\subsection{Distributions}

Other than extracting singular value properties like the discussed so far, we are also investigating ways to extract more valuable information from the blockchain by tracking the activity of the crypto accounts in higher detail. This is achieved by creating account distributions- 2D matrices that visualize account activity based on multiple account features. These distributions contain spatial value, which Convolutional networks can take advantage of. 

Let us introduce some common definitions: $scl$ as an array of scale functions, $feat$ as an array of functions that return an account feature, and $mx$ as an array of constants.

Possible values for $scl_i$ include $\log_2$ and $\log_{1.2}$. Possible account features ($feat_i$) are defined in Table \ref{account_feature_table}.

\begin{table}[h]
\centering
\begin{tabular}{lp{6cm}}
Feature & Description \\\hline
balance & Account balance, measured in $wei$ ($10^{18}$ $wei$ = 1 $ETH$). \\
lastSeen & Amount of seconds since the account's last participation in a transaction. \\
volumeIn & Amount of received value in the last tick, in $wei$. \\
volumeOut & Amount of sent value in the last tick, in $wei$. \\
transactionN & Amount of transactions where the account as either a receiver or a sender.\\
ERC20 & Amount of ERC20 token operations in the last tick (Ethereum contracts only) \\
\end{tabular}
\caption{\label{account_feature_table}The possible account feature functions.}
\end{table}

\subsection{Account balance distribution}
\label{account_balance_distribution}

This distribution visualizes summarized recent account activity in terms of the exchanged volume and amount of transactions, distributed based on balance groups.

Let us define $scl_0 = \log_2 \; mx_0=10^{26} \; feat_0=volumeIn \; feat_1=volumeOut \; feat_2=transactionN \; groupN = \lfloor\ scl_0(mx_0)\rfloor \; featN=3 $, $S$ as the accounts that have participated in a transaction in the current market tick, and $distribution$ as a matrix of shape $(featN, groupN)$.

For $acc \in S$:

\hspace{3em} $gr = \min(\lfloor scl_0(balance(acc))\rfloor, groupN-1)$

\hspace{3em} For $x \in [0, featN)$:

\hspace{6em} $distribution_{x, gr} \; += feat_x(acc)$

$distribution = scl_0(distribution)$

The final operation is to scale the large values of volumeIn and volumeOut.

Figure \ref{account_balance_graph} contains an example of $2$ such distributions.

\begin{figure}[h]
\centering\includegraphics[width=\graphwidth]{assets/distributions/accountBalanceDistribution_log1_2}\\
\centering\includegraphics[width=\graphwidth]{assets/distributions/accountBalanceDistribution_log2}
\caption{Examples with $scl_0=\log_{1.2}$ (up) and $scl_0=\log_{2}$ (down). We observe how the summarized account trade activity changes in the different balance groups.}
\label{account_balance_graph}
\end{figure}

\subsection{Account number distributions}
\label{account_number_distribution}

These multivariate distributions represent how the accounts are clustered based on 2 of their account features.

The process of creating an account number distribution is described as follows:
\vspace{1em}

Repeat for $x = 1$ and $x = 2$:

\hspace{3em} $groupN_{x} = \lfloor scl_{x}(mx_{x})\rfloor$

For $acc \in S$, where $S$ is a chosen subset of (or all) accounts, do:

\hspace{3em} Repeat for $x = 1$ and $x = 2$:

\hspace{6em} $group_{x} = \min(\lfloor scl_{x}(feat_{x}(acc))\rfloor, groupN_{x}-1)$

\hspace{3em} $distribution[group_1, \; group_2] \; += 1$

Finally, for every value, do:

\hspace{3em} $distribution = \log_2(distribution)$

The final $\log_2$ scaling is to mitigate the uneven distribution of accounts. The possible options for the $feat$ functions are defined in Table \ref{account_feature_table}. Some configurations of distributions are presented in Table \ref{account_number_table} and are later referred to in the experiments.

\begin{table}[h]
\centering
\setlength\tabcolsep{1.5pt} % TEMPORARY FIX
\begin{tabular}{lrrrrrrrp{5cm}}
$N$ & $S$ & $feat_1$ & $feat_2$ & $scl_1$ & $scl_2$ & $mx_1$ & $mx_2$ \\\hline
1 & all & balance & lastSeen & $\log_{1.2}(\lfloor x / 10^{17} \rfloor)$ & $\log_{1.2}$ & $10^{7}$ & $20736e3$ \\
2 & contracts & balance & lastSeen & $\log_{1.2}(\lfloor x / 10^{17} \rfloor)$ & $\log_{1.2}$ & $10^{7}$ & $20736e3$ \\
3 & contracts & volumeIn & ERC20 &  $\log_{2}(\lfloor x / 10^{17} \rfloor)$ & $\log_{2}$ & $10^{7}$ & $262144$ \\
\end{tabular}
\caption{\label{account_number_table}The configurations for account number distributions. The balances and transfers, measured in wei, are scaled to larger units ($10^{17}$ $wei$ = $0.1$ $eth$) to reduce noise.}
\end{table}

Consequently, we refer to the distribution configurations as follows: balanceLastSeenDistribution (N=1), contractBalanceLastSeenDistribution (N=2), and contractVolumeInERC20Distribution (N=3). Example distributions are visualized in Figure \ref{account_number_example}.

\begin{figure}[h]
\centering\includegraphics[width=0.8\graphwidth]{assets/distributions/balanceLastSeenDistribution_log1_2}\\
\centering\includegraphics[width=0.7\graphwidth]{assets/distributions/contractVolumeInERC20Distribution_log2_v2_stateless}
\caption{
\textbf{balanceLastSeenDistribution (up)}: we observe the difference in activity of the most active accounts (left) and richest accounts (down). The empty lines are seen because $\lfloor\log_{1.2}(x)\rfloor \notin \{1, 2, 4, 5\}$ for all $x$.
\if\showlinks1
User behavior and major market movements are more effectively seen in a time-lapse video of the distribution values (\href{https://youtu.be/Dwwnxn1j6AQ}{https://youtu.be/Dwwnxn1j6AQ}).
\fi
\textbf{contractVolumeInERC20Distribution (down)}: we observe the different proportions of a crypto contract being used ($X$) and the amount of funds received from it ($Y$).
}
\label{account_number_example}
\end{figure}

\section{Generation of a dataset}

A dataset is a set of samples, containing inputs (normalized property data) and expected outputs (prediction target). The concepts and methodologies behind dataset generation are defined in the following subsections.

\label{dataset-generation}

\subsection{Prediction target}
%not sure if 51% attacks should be mentioned
The prediction target is the future value a chosen target property. Predictions are for the duration of one market tick. Examples of a prediction target include relative price fluctuations, amount of new accounts, trade volume, transaction count and network clogging (a serious issue in the light of recent events \cite{blockchain-clogging}).
%or possibly attempts of 51\% attacks \cite{51attack}.

Our experiments will be mainly focused on predicting price movements and new accounts.

\subsection{Normalization}
\label{normalization}

Every property in a dataset is a different time series and is normalized separately with a chosen algorithm (among those defined in Secion \ref{normalization_bg}). A method to automatically determine the algorithm for a given property is called $prop$, which uses $basic$ scale if the property values are absolute and $around\_zero$ scale otherwise.

Most of the algorithms scale on the basis of $\min$ and $\max$ bounds, hence future values may not fit that initial scale. The problem is mitigated if the normalized values are relative, which has also resulted in lower overfit and higher prediction accuracy in our experiments.
%the below technique is not used
%We also use a technique called normalization space overprovisioning, which increases the initial $\min$ and $\max$ values by a given percentage so that future values are more likely to fit.
%The problem of future values can be solved completely by using $local$ normalization, but that is not the best algorithm in all cases.
%All of the aforementioned methods to deal with the problem can be used in conjunction with each other.

\subsection{Dataset models}
\label{dataset-models}
The dataset samples (input-output pairs) are created using a sliding window with a size of $wn$ and step increments of $1$ over a chosen set of normalized property values. Let us define a property's values as $prop_y$, where $y < propN$, a specific value in a property time series as $prop_{y,x}$, and $prop_{t}$ as the prediction target.

%$step=0$

For $x \in [0, wn-1]$, do:

\hspace{3em} For $y \in [0, propN-1]$, do:

\hspace{6em} $win_{x,y} = prop_{y,x+step}$

\hspace{0em} $tar = prop_{t, wn+step}$

Where $win$ is the window (unstructured dataset input), $tar$ is the expected output, and $step$ is incremented for each window.

In order to combine multiple normalized properties in a single dataset, we need the following models that define how their values are arranged in N-dimensional space.

\subsubsection{Matrix model}

Based on the LSTM network's 2D input shape, the matrix model defines one dataset sample as being the same as its corresponding $win$, without modifying its structure in any way.

Table \ref{matrix_model_table} visualizes the structure of a dataset sample.

\begin{table}[h]
\centering
\begin{tabular}{lrrr}
Property & Value $0$ & Value $1$ & ... Value $wn-1$ \\\hline
Close value & 349\$ & 358\$ \\
Number of TXs & 2876 & 1583 \\
Operations with Contracts & 459 & 508 \\
\end{tabular}
\caption{\label{matrix_model_table}Example of a matrix model dataset sample.}
\end{table}

\subsubsection{Stacked layers model}
\label{stacked-model}

%\begin{wrapfigure}{R}{0.5\graphwidth}
\begin{figure}
%\centering\includegraphics[width=\linewidth]{assets/stacked_model}
\centering\includegraphics[width=0.5\graphwidth]{assets/stacked_model}
\caption{Visualized sample of the stacked layers model, where $wn=3$ and the chosen properties consist of balanceLastSeenDistribution.}
\label{stacked_model_example}
\vspace{-0pt} %workaround, because wrapfigure hates the float package
%\end{wrapfigure}
\end{figure}

A given set of property values (a column in $win$) has shape $(v_1, v_2, wn)$, where $v_1 = 1$ and $v_2 = 1$ for all properties but the distributions (discussed in Sections \ref{account_balance_distribution} and \ref{account_number_distribution}); these properties with windowed values of 3D shape can't be modeled by a matrix. The stacked layers model is a 3D structure that matches input shape for the Convolutional Neural Network and allows modeling of 3D shaped property windows, preserving their spatial value. 

The model defines a 3D matrix $mat$ of shape $(values_1, values_2, wn)$. A dataset sample $mat$ is created as follows. For every set of windowed property values $vals$:

$$mat_{s_1 + (0 \; to \; v_1), s_2 + (0 \; to  \; v_2), 0 \; to \; wn} = vals_{0 \; to \; v_1, 0 \; to \; v_2, 0 \; to \; wn}$$

Where $s_1$ and $s_2$ are set to the smallest integers where no values of other previously assigned properties are overridden. A visualized sample produced this model is seen in Figure \ref{stacked_model_example}.

\vspace{1pt} %to move the title of the next section to the next page


==> front/predictor_abstract_en.tex <==
%Predicting the future is impossible. Yet, the better estimation we have about the future, the more power we h	ave to make the most optimal decision in the present. 

Blockchain technology shows significant results and huge potential for serving as an interweaving fabric that goes through every industry and market, allowing decentralized and secure value exchange, thus connecting our civilization like never before.

The standard approach for asset value predictions is based on market analysis with an LSTM neural network. Blockchain technologies, however, give us access to vast amounts of public data, such as the executed transactions and the account balance distribution. We explore whether analyzing this data with modern Deep Leaning techniques results in higher accuracies than the standard approach.

%In our paper we explore how modern Deep Learning techniques can be applied to predict future facts about the Ethereum blockchain. Specifically, we are interested if blockchain's public raw data, such as the transaction count and the account balance distribution, can be used to predict other measures like the number of new accounts created and the market price per ETH token.

During a series of experiments on the Ethereum blockchain, we achieved $4$ times error reduction with blockchain data than an LSTM approach with trade volume data. By utilizing blockchain account distribution histograms, spatial dataset modeling, and a Convolutional architecture, the error was reduced further by 26\%.

The proposed methodologies are implemented in an open source cryptocurrency prediction framework, allowing them to be used in other analysis contexts.

%Moreover, we have developed a reusable framework providing data gathering, processing, and storing functionality for performing Deep Learning experiments over blockchain data.
%Our future plans are towards automating neural network architecture and meta-parameter optimization tasks through training controller Machine Learning models on these tasks. Since the Ethereum network already utilizes a great amount of GPU processing power, which might become obsolete due to the adoption of a Proof-of-Stake algorithm, we believe that 2018 presents a unique opportunity for achieving an exascale decentralized supercomputer, dedicated to training AI.

%----------------

%The crypto-asset markets are public, decentralized and transparent by definition. In our research, we explore the new kind of data available on the Ethereum blockchain in efforts to create an accurate prediction strategy using deep neural networks. We gather our data from multiple sources and extract the most important data points (properties) from it. Other than basic properties, we explore different methods to create complete network state snapshots by generating multiple values that are specifically ordered in time and space. We have proposed multiple methods to model a dataset by aligning the property values differently in multidimensional space. We have built neural network architectures that are based on basic deep, Long Short-Term Memory (LSTM) and Convolutional networks. We ran different experiments with each one of them and with different datasets. Because the convolutional network is able to extract meaning from spatially related data, it performed far superior than any other model we have tried. Due to its high volatility, Ethereum has proven difficult to predict. Despite that, our results have shown a strong correlation between blockchain and price data. We should focus most of our efforts in perfecting the quality of our dataset, before tweaking the network architecture. We have found that increasing the spatial value in our dataset also increases the prediction accuracy.

%For our experiment, we have created and documented a flexible framework that allows the prediction of any cryptocurrency on the base of any data.


==> predictor_content_en.tex <==
\section{Introduction}

Cryptocurrencies, the decentralized new ways of exchanging value, are gaining a lot of interest recently with the emergence of Bitcoin, Ethereum, and hundreds of other cryptoassets with total value that recently exceeded \$500 billion. Unlike the traditional markets, where all the data about the market and the trading itself are centralized and controlled by gatekeeper organizations, the cryptoasset markets are public, decentralized and transparent by definition.

%hypothesis
The new kind of data available on the blockchain can be analyzed together with standard market information in an attempt to predict future market movements.

%research goal
Our goal is to explore whether we can utilize the abundant blockchain data using modern Deep Learning techniques to estimate future facts about cryptoassets.

%say that blockchain is volatile and price data just won't cut it - comparison with world economical crisis
%Most forex and stock market predictions are based solely on previous price points. Similar prediction strategies, however, perform very poorly in the volatile cryptocurrency markets. To combat that we can analyze the public blockchain data, in addition to financial data, in an attempt to predict the future values.

%something about the framework?
%state how much is lost by volatility

%\subsection{Project Goals}

In this paper, we are introducing a set of methodologies for the cryptocurrency prediction problem and demonstrate their performance on the Ethereum ($ETH$) cryptocurrency \cite{yellowpaper}. First, raw blockchain and financial data is collected (Secton \ref{data-sources}), which is used in different feature extraction algorithms (Section \ref{property-generation}). The features are compiled into a dataset using different modeling techniques (Section \ref{dataset-generation}). Custom neural architectures are trained, evaluated and compared on their predictive performance (Section \ref{networks} and \ref{experiments}).

%We have concluded that the Ethereum blockchain ($ETH$) \cite{yellowpaper} is probably the most difficult to predict, due to its large and versatile user base. Some of its use cases include financial transactions, secure voting, autonomous organizations, company management, freedom of speech networks, online games, crowdfunding, speculation, and more. This stochastic environment will be the best to show the true performance of our prediction strategies, which can later be migrated to less noisy blockchains, like Bitcoin.

\subsection{Related work}

Projects about cryptoasset market predictions have emerged in the past, including a paper by a Stanford University team \cite{stanford-predictions} and two more recent Github projects \cite{bitpredict} \cite{deep-learning-bitcoin}. All of them focus primarily on Bitcoin price estimations, do not explore the rich publicly available blockchain data in depth, and do not use or have not disclosed sophisticated deep learning techniques for their estimations.

\input{common_content.tex}


\section{Generated datasets}
\label{generated-datasets}

The experiment setup includes a number dataset configurations. The interval of the datasets is from 2017-03-01 to 2017-11-01. This range contains the largest fluctuations in Ethereum's history, the widespread media hoax about Ethereum \cite{vitalik-death}, and the rise of ICOs \cite{ico}.

%we don't include any stateful LSTM experiments. No need to specify warmup dataset
Each complete dataset is split on $train$ and $test$ datasets.
%The first month of the range is reserved for the $warmup$ dataset. This part is only utilized in our stateful LSTM experiments and is used to initialize the network state before training or evaluation.
The first 7 months of the range build the $train$ dataset, on the basis of which the neural network is trained. The last month is utilized by the $test$ dataset, used for evaluation of the already trained network. 

% !!! I don't like how we refer to datasets here as complete, but as a matter of fact, they're not (wn, Norm & target are specified later).

The dataset configurations are defined in Table \ref{dataset_table}. Window size ($wn$), prediction target and the normalization ($Norm$) are specified later in the experiments. As datasets $1$ to $4$ do not include blockchain data, they are used as a baseline for comparison.

%multiple prediction targets?
\begin{table}[h]
\centering
\begin{tabular}{lp{6.0cm}r}
setN & Properties in dataset & Model \\\hline
1 & volumeFrom, volumeTo & matrix\\
2 & volumeFrom\_rel, volumeTo\_rel & matrix\\
3 & highPrice, volumeFrom, volumeTo & matrix\\
4 & highPrice\_rel, volumeFrom\_rel, volumeTo\_rel & matrix\\
5 & accountBalanceDistribution & matrix\\
6 & balanceLastSeenDistribution & stacked\\
7 & contractBalanceLastSeenDistribution & stacked\\
8 & balanceLastSeenDistribution, contractBalanceLastSeenDistribution, contractVolumeInERC20Distribution, accountBalanceDistribution & stacked\\
\end{tabular}
\caption{\label{dataset_table}The dataset definitions.}
\end{table}

\texcomment{
\section{The genetic engine}
\label{genetic-framework}

Deep models usually have hundreds of hyper- and meta-parameters regarding the neural architecture, training parameters and dataset configuration that have to be individually tuned. The address space for possible configurations is too large compared to what we are able to optimize by hand. Our prediction framework allows for automatic tuning of some hyper-parameters by repetitive training, evaluation and respective parameter adjustments. This technique has been applied to our experiments. To automate the process further, we have chosen to create a genetic engine that aims to automate neural architecture search, hyper-parameter and dataset configuration by evolving agent machine learning models to accomplish a given predictive task.

An agent represents a deep network with its training parameters. An agent is created from a genome, consisting of a set of chromosomes. Each chromosome represents an array of integers with length based on the chromosome type. Example types include input data configuration, training parameters and a deep network layer with its their parameters (ex. $Conv2d$, $LSTM$). We have created a $JSON$ specification that allows the notion of any deep network configuration, and a converter that creates said $JSON$ from a genome. The output $JSON$ is passed to a parser that creates and returns the deep model, ready for training. 

\begin{figure}
\centering\includegraphics[width=\graphwidth]{assets/genetic_engine}\hfill
\caption{The structure of the genetic engine}
\label{genetic-framework-scheme}
\end{figure}

Please refer to Figure \ref{genetic-framework-scheme}. Initially, a population of $n$ individuals (genomes) is created with random chromosomes. Most chromosome values have limits (ex. the size of a deep layer cannot be a negative value). Each individual is passed through an initial check that modifies the chromosomes to be within all limits. Afterwards, the individuals are converted to our $JSON$ spec and parsed to deep models. Should the parsing stage fail (ex. an invalid combination of layers), the individual is killed. Reinforcement learning agents are created from these models and trained to emit signals of ``buy'' and ``sell'' for trading.
The properties included in the dataset of an individual are denoted in its genome. After training, each agent is evaluated and ranked with a fitness score based on their trading performance on a test dataset.

A set of new individuals is created via random binary mutations in the chromosome values, random chromosome addition/removal, Two-point crossover \cite{twopoint-crossover} and Uniform crossover \cite{uniform-crossover} from two parents, which are selected via Fitness proportionate selection and Tournament selection. The top $x\%$ of performing individuals are not mutated, while the worst ones are removed to keep the population number stable. The resulting set of individual's genomes are converted to $JSON$ and an agent is created for each one, which is trained afterwards. This algorithm is repeated until individuals with desirable performance are found.

The genetic engine is still under development and the following results and neural architectures do not take advantage of it yet.
\if\showlinks1
The engine is open source and available under \href{https://github.com/obecto/gattakka}{the following address: https://github.com/obecto/gattakka}
\fi
}

\section{Neural Network architectures}
\label{networks}

The experimental setup includes a Long Short-Term Memory (LSTM) \cite{LSTM} and a Convolutional (CNN) \cite{cnn} models. Their network architectures are described in Figure \ref{models}. 

The LSTM model, trained with datasets 1 to 4, is used as a baseline for comparison of the blockchain data approach. 

\begin{figure}[h]
\centering
\includegraphics[width=1.05\graphwidth]{assets/architectures_short_nodnn}
\caption{The architecture of the LSTM and Convoluitonal models respectively}
\label{models}
\end{figure}

\section{Experiments}
\label{experiments}

We have performed hundreds of experiments with different dataset configurations and neural architectures. Out of those, the best ones are selected and grouped per prediction target.

The performance measurements are taken after inverse normalizing the network output and are therefore normalization independent. All measurements besides $sign$ rely on the distance between the curves for prediction and actual values and are therefore directly incomparable between experiments with different targets. 

The experimentally selected optimal training parameters include batch size of $16$, $10^{-5}$ learning rate, and training via the Adam optimizer \cite{adam}. All networks are trained with these parameters.

\subsection{Predicting value ($highPrice$)}
\label{highPrice_exp}

\begin{table}[h]
\centering
\begin{tabular}{lrrrrrrr}
$N$ & $setN$ & $win$ & $Norm$ & $Netw$ & $RMSE$ & $R^2$ & $sign$ \\\hline
%matrix-volumeFrom_rel,volumeTo_rel-highPrice-pixel-24w.pickle.pickle
1 & 2 & 24 & image & LSTM & 90.4185 & 0.9131 & 0.5258\\
%matrix-highPrice,volumeFrom,volumeTo-highPrice-property-8w.pickle.pickle
2 & 3 & 8 & prop & LSTM & 5.1060 & 0.9997 & 0.5095\\
%matrix-accountBalanceDistribution-highPrice-pixel-24w.pickle.pickle
3 & 5 & 24 & image & LSTM & 21.9306 & 0.9948 & 0.5054\\
%stacked-balanceLastSeenDistribution_cpp_log2-highPrice-pixel-104w.pickle.pickle
4 & 6 & 104 & image & CNN & 16.2167 & 0.9972 & 0.5115\\
%stacked-balanceLastSeenDistribution_cpp_log2-highPrice-pixel-8w.pickle.pickle
5 & 6 & 8 & image & CNN & 21.2845 & 0.9951 & 0.5033\\
%stacked-contractBalanceLastSeenDistribution_log2_v2-highPrice-property-104w.pickle.pickle
6 & 7 & 104 & prop & CNN & 83.1030 & 0.9265 & 0.5290\\
%stacked-contractBalanceLastSeenDistribution_log2_v2-highPrice-property-24w.pickle.pickle
7 & 7 & 24 & prop & CNN & 82.2199 & 0.9280 & 0.5367\\
\end{tabular}
\caption{\label{highPrice_table}Results for target $highPrice$. The measurements are the best ones from all training epochs.}
\end{table}

While the error scores on experiment $2$ seem impressive, the network cheats by returning the inputted previous price data, instead of making an actual prediction. Experiment $1$ does not input such information and forces the network to find an accurate solution. This can be seen in Figure \ref{1_2_highPrice}. In order to avoid such scenarios, the input data in all CNN experiments omits previous prices.

\begin{figure}[h]
\centering
\includegraphics[width=\graphwidth]{assets/1_highPrice}\\
\includegraphics[width=\graphwidth]{assets/2_highPrice}
\caption{$highPrice$: The test results of exp $2$ (bottom) and exp $1$ (top). We observe how exp $2$ achieves high accuracies by copying the previous price as a prediction and the result of omitting that data.}
\label{1_2_highPrice}
\end{figure}

Exp $3$ utilizes blockchain data and reaches an error reduction of 4 times compared to that of exp $1$. Despite not using any market data, the network is able to predict multiple major market movements (Figure \ref{3_highPrice}).

\begin{figure}[h]
\centering
\includegraphics[width=\graphwidth]{assets/3_highPrice_big}
\caption{$highPrice$: The test results of exp $3$. On multiple occasions, we observe valid reactions to major market movements.}
\label{3_highPrice}
\end{figure}

Exp $4$ includes more valuable blockchain data and combined with CNN results in the lowest error scores for this target (26\% lower than that of exp $3$).

The high errors on experiments $6$ and $7$ may indicate that $prop$ normalization is not suitable for distributions.

\subsection{Predicting relative value ($highPrice\_rel$)}

\begin{table}[h]
\centering
\begin{tabular}{lrrrrrrr}
$N$ & $setN$ & $win$ & $Norm$ & $Netw$ & $RMSE$ & $R^2$ & $sign$ \\\hline
%matrix-volumeFrom,volumeTo-highPrice_rel-property-104w.pickle.pickle
1 & 1 & 104 & prop & CNN & 2.3652 & -0.0031 & 0.5502\\
%matrix-highPrice_rel,volumeFrom_rel,volumeTo_rel-highPrice_rel-pixel-104w.pickle.pickle
2 & 4 & 104 & image & CNN & 2.3019 & 0.0498 & 0.4932\\
%stacked-contractBalanceLastSeenDistribution_log2_v2-highPrice_rel-pixel-24w.pickle.pickle
3 & 7 & 24 & image & CNN & 2.2825 & 0.0513 & 0.5340\\
%stacked-balanceLastSeenDistribution_cpp_log2,contractBalanceLastSeenDistribution_log2_v2,contractVolumeInERC20Distribution_log2_v2_stateless,accountBalanceDistribution-highPrice_rel-pixel-8w.pickle.pickle
4 & 8 & 8 & image & CNN & 2.2878 & 0.0461 & 0.5512\\
%stacked-balanceLastSeenDistribution_cpp_log2,contractBalanceLastSeenDistribution_log2_v2,contractVolumeInERC20Distribution_log2_v2_stateless,accountBalanceDistribution-highPrice_rel-property-104w.pickle.pickle
5 & 8 & 104 & prop & CNN & 9.1956 & -14.2060 & 0.5466\\
\end{tabular}
\caption{\label{highPrice_rel_table}Results for target $highPrice\_rel$.}
\end{table}

Because the next relative change, as a value, is too different from the last relative change, a network cannot increase its score without predicting accurately. This explains the small error difference between exp $1$ (volume data) and $2$ (price \& volume data).

Experiment $4$ utilizes 4 blockchain distributions and results in the lowest error and highest sign accuracy. However, when observing the prediction plot (Figure \ref{4_highPrice_rel}), the network is seen as less confident in its predictions. This may be mitigated with further network architecture and hyperparameter optimization.
% IS THIS LAST SENTENCE FOR HERE?

\begin{figure}[h]
\centering
\includegraphics[width=\graphwidth]{assets/4_highPrice_rel_big}
\caption{$highPrice\_rel$: The test results of exp $4$. The small $\sigma$ of the predictions suggests lower prediction confidence.}
\label{4_highPrice_rel}
\end{figure}


\subsection{Predicting user growth ($uniqueAccounts\_rel$)}

\begin{table}[H]
\centering
\begin{tabular}{lrrrrrr}
$N$ & $setN$ & $win$ & $Norm$ & $Network$ & $RMSE$ & $R^2$ \\\hline
%matrix-volumeFrom_rel,volumeTo_rel-uniqueAccounts_rel-property-104w.pickle.pickle
1 & 2 & 104 & prop & LSTM & 1139.972426 & 0.737456\\
%matrix-volumexFrom,volumeTo-uniqueAccounts_rel-property-104w.pickle.pickle
2 & 1 & 104 & prop & LSTM & 718.971374 & 0.895567\\
%stacked-contractBalanceLastSeenDistribution_log2_v2-uniqueAccounts_rel-pixel-8w.pickle.pickle
3 & 7 & 8 & image & CNN & 812.303885 & 0.864637\\
%stacked-balanceLastSeenDistribution_cpp_log2-uniqueAccounts_rel-pixel-24w.pickle.pickle
4 & 6 & 24 & image & CNN & 639.336022 & 0.916289\\
%stacked-balanceLastSeenDistribution_cpp_log2,contractBalanceLastSeenDistribution_log2_v2,contractVolumeInERC20Distribution_log2_v2_stateless,accountBalanceDistribution-uniqueAccounts_rel-pixel-8w.pickle.pickle
5 & 8 & 8 & image & CNN & 622.716696 & 0.920449\\


\end{tabular}
\caption{\label{uniqueAccounts_rel_table}Results for target $uniqueAccounts\_rel$.}
\end{table}

This set of experiments aims to demonstrate how blockchain data can be used to predict other facts about the blockchain, like how the amount of unique users will grow.

Sign accuracy is irrelevant in this case, as the number of\\ $uniqueAccounts$ always increases.

When predicting blockchain facts, it is not a surprise that the experiments with market data ($1$ and $2$) result in the lowest accuracies. Experiment $5$ (Figure \ref{5_uniqueAccounts_rel}) yields impressive results in all measurements, which is likely due to the 4 distributions in its dataset.

\begin{figure}[H]
\centering
\includegraphics[width=\graphwidth]{assets/5_uniqueAccounts_rel_big}
\vspace{-0em}
\caption{$uniqueAccounts\_rel$: The test results of exp $5$. The prediction curve follows the actual values relatively accurately.}
\label{5_uniqueAccounts_rel}
\end{figure}


\section{Results}

Through the experiments, we have observed the problem from different angles, by training different networks, dataset configurations, and evaluation metrics.

The results have shown that Ethereum is too volatile to be predicted based solely on market data.

The best overall results are achieved using the proposed blockchain analysis approach, confirming our initial hypothesis that this kind of data can assist predictions. The approach has demonstrated effective $4$ times reduction in error scores compared to only trade volume data. With the proposed Convolutional architecture, spatial account distributions, image normalization, and spatial dataset modeling, the error was additionally reduced by 26\%. Training times were also reduced by a factor of 10. 

Basic blockchain properties (as defined in Table \ref{properties}) have demonstrated to be inefficient for the predictive task. These findings are consistent with the lower hourly prediction scores on the Bitcoin trading research by the Stanford research group \cite{stanford-predictions}.

The spatial distributions have been consistently linked to the highest accuracy results, as they are able to analyze the blockchain raw data in more depth than other approaches.

The overall best dataset found combines all 4 of the spatial distributions (Number $8$ in Table \ref{dataset_table}), modeled by the Stacked layers model (Section \ref{stacked-model}). The best found prediction target is relative high price, which forces the models to find the best possible predictive strategy. 

The overall most accurate neural network is the proposed Convolutional model. Its ability to extract spatial meaning from the data likely contributes to its success in the distributions.

%UNNEEDED
%We recommend batch size of 16, which provides balance between training times and network generalization. There are methods to increase accuracy with large batches \cite{accurate-large-batch}, but a smaller batch is always better in terms of generalization.

The best blockchain approach includes many parameters that have to be further explored before we can state the extent to which blockchain data can assist predictions.

\if\showtech{1}

\section{Technical implementation}

For our experiment, we have created and documented a robust framework which can be used as a foundation for the development and training of models that predict facts about any blockchain and based on any data. All the referenced in this paper properties, dataset models, normalization strategies and the aforementioned techniques are all included in the source code provided with the open source framework. 

The framework is split into multiple tools for managing data download and storage, property generation, dataset generation, and neural network training and evaluation:

\begin{itemize}
\item \textbf{Dataset extraction module}: responsible for connection to data providers (like the ones discussed in Section \ref{data-sources}), download, validation of integrity, and storage of the raw data.

\item \textbf{Data storate module}: reads and post-processes the raw data by filtering out unimportant for our research data and saving the rest as a time series in a database. For fast retrieval by date interval, the data is split by a chunking algorithm.

\item \textbf{Property generation module}: generates and stores time series of property values (discussed in Section \ref{property-generation}) by utilizing the raw time series data.

\item \textbf{Dataset generation module}: normalizes the property values and applies a chosen dataset model to generate a dataset (the process is described in Section \ref{dataset-generation}).

\item \textbf{Training and evaluation module}: trains and evaluates a chosen neural architecture on a specified dataset (our proposed architectures are in Section \ref{networks} and our error measures are described in Section \ref{measures}).
\end{itemize}


\subsection{Automated tests}

We have implemented unit and integration tests for all of our tools, where applicable. This is done to ensure that the dataset generated by those tools is always with the expected and true values.


\section{Technologies}

\begin{enumerate}
\item \textbf{JavaScript} is used for the data extraction module;
\item \textbf{Web3 API} allows the extraction of blockchain data from a local running Ethereum node;
\item \textbf{Node.js} creates connections to other APIs for the rest of our raw data;
\item \textbf{Python} is used for all other modules;
\item \textbf{Pandas} provides high-performance data structures and data analysis tools for Python;
\item \textbf{MongoDB} is the database we use to store our data throughout all stages of data processing;
\item \textbf{Arctic} is a high performance datastore for numeric and time-series data used in hedge funds;
\item \textbf{Tensorflow} is the Deep Learning library most commonly used in Deep Learning research and development;
\item \textbf{Keras} is a frontend framework for a backend (like Tensorflow) that allows quick development of neural network architectures;
\item \textbf{Scala} is used in the core of the genetic framework;
\item \textbf{Akka} is a framework for the actor model, implemented in the genetic framework, allowing scaling of agent optimization tasks over multiple computing nodes simultaneously.
\end{enumerate}

\fi

\if\showlinks1
\section{Cryptocurrency prediction framework}

The technical implementation of the data processing, dataset generation and neural network evaluation processes is developed into an open source Cryptocurrency prediction framework. The framework allows for the prediction of a chosen cryptocurrency on the basis of user-defined property extraction and neural algorithms. \href{https://github.com/Zvezdin/blockchain-predictor}{The framework can be accessed at: https://github.com/Zvezdin/blockchain-predictor}

The repository includes the necessary technical documentation for the reproduction or improvement of our experimental results.

All trained model weights, detailed training histories, and performance visualizations, are available \href{https://goo.gl/uBQn4p}{here: https://goo.gl/uBQn4p}.

\section{Future work}

Throughout the research, we have evaluated not only a number of Deep Learning models but we have also built a reusable framework for data gathering, processing and storage of blockchain and market data. Once we had this framework, most of our actual research work was reduced to trying different network architectures and meta-parameters. While this process alone was challenging and demanding of both deep knowledge and creative thinking, we are excited by the possibilities to experiment with automating it. 

Two recent publications by Google Research \cite{automl-genetic} \cite{automl-rl} show that given enough computing power, we can create a ``controller'' algorithm which produces model designs for predicting the CIFAR10 dataset \cite{cifar-10}, with performance on par with state-of-art models designed by humans. The process is called neural architecture search (NAS). The authors emphasize the enormous computational power required for achieving these results which was in order of $10^{20}$ computation. For comparison, most estimations about the computational power of the human brain are for between petascale ($10^{15}$) and exascale ($10^{18}$) operations per second \cite{brain-processing-power}.

We are interested in exploring NAS methodologies in order to find the most optimal neural configuration for blockchain data analysis.

Furthermore, we hope to develop a scalable decentralized architecture which allows remote nodes to provide computing power to ``controller'' algorithms for evaluating individual Deep Learning models. In such a system, Ethereum smart-contracts can be utilized to implement a decentralized marketplace for neural network model training and optimization. 

Blockchain mining, which consumes enormous amounts of electrical power \cite{electricity-for-mining}, might soon become obsolete due to the adoption of more efficient consensus algorithms like Proof-of-Stake. This presents an unique opportunity to utilize the abundant GPU mining resources for more reasonable work, like training Deep Learning models.

%NEEDED?
%We are excited to work towards our new research goal during 2019, since this year might present a unique opportunity to build the first decentralized exascale supercomputer dedicated for training AI.


\section{Conclusion}

%NEEDED?
Blockchain technology enables a new class of tradable cryptotoken assets, thus creating new kinds of markets with numerous new use cases. Due to their decentralized and open nature, public blockchains provide an abundance of market-related data that has never been available before. Having every account balance and every transaction visible encourages us to seek a holistic view on the blockchain dynamics.

In our research project, we have evaluated different Deep Learning methods at their ability to find patterns in the Ethereum blockchain data and provide estimations about future measurements of the blockchain assets, including their market price. To facilitate our experiments, we have implemented a data gathering, processing, and storing framework that enabled us to deal with the enormous amount of data on the blockchain (more than 1000GB) and efficiently produce datasets for training.

We have tested both Recurrent and Convolutional models with different data sets and prediction targets. The most interesting results came from our Convolutional models which were working on account distribution histograms with one, two, and three dimensions. These histograms serve as ``pictures'' of the blockchain in a certain period of time and when we observe
\if\showlinks1
a \href{https://youtu.be/Dwwnxn1j6AQ}{time-lapse video of such 2D histograms (https://youtu.be/Dwwnxn1j6AQ)},
\else
their historical values,
\fi we can clearly see patterns that correlate to major market moves. After experimenting with these novel blockchain data representations, we found that Convolutional Deep Learning models are capable of providing estimations for the ETH token price based solely on such histogram data. Still, we believe that better results can be achieved by further optimizations of the model architectures and meta-parameters.

Since the search space for such optimizations is enormous, we will be focusing on creating efficient NAS approaches that automate the search process. We will also be investigating different ways in utilizing independent GPU resources in the common goal of finding a more efficient neural network.


%TODO: Wait for kosta reply
%\section{Acknowledgements}

%We would like to thank HSSIMI for allowing us to start our research at the Summer Research School.
